RanDeS: Randomized Delta Superposition for Multi-Model Compression

From a multi-model compression perspective, model merging enables memory-efficient serving of multiple models fine-tuned from the same base, but suffers from degraded performance due to interference among their task-specific parameter adjustments (i.e., deltas). In this paper, we reformulate model merging as a compress-and-retrieve scheme, revealing that the task interference arises from the summation of irrelevant deltas during model retrieval. To address this issue, we use random orthogonal transformations to decorrelate these vectors into self-cancellation. We show that this approach drastically reduces interference, improving performance across both vision and language tasks. Since these transformations are fully defined by random seeds, adding new models requires no extra memory. Further, their data- and model-agnostic nature enables easy addition or removal of models with minimal compute overhead, supporting efficient and flexible multi-model serving.

==> sec/sections/0_notes.tex <==
\section{Internal Notes}
"Everything should be made as simple as possible, but not simpler".

\begin{enumerate}
    \item Have a super clear and well-motivated problem setup. Think about the big picture, situate your work at an important intersection of research trends with big and common interest across the whole AI community.
        \begin{enumerate}
            \item Move the centre away from niche area (model merging) and to hot topics (model compression).
            \item Potential use cases for programmatic foundation models like VisProg, ViperGPT, HuggingGPT to save and use neural primitives more efficiently.
        \end{enumerate} 
    \item Extensive experiments and perfect writing.
    \begin{enumerate}
        \item Finish all experiments and writing three weeks before deadline to have ample time for iterative refinement until the paper is absolutely perfect (minimal, elegant, and intriguing).
    \end{enumerate}
\end{enumerate}

\textbf{Overview.} Level up the entire model merging field with principled methods called model superposition. It encompasses a few key ingredients: i) Chop up weight matrices into atomic blocks; ii) Group similar blocks together; iii) Introduce redundant blocks to absorb interference; iv) Superpose blocks together with block-specific context matrix; v) Retrieve each block with the inverse context matrix.

It's a simple but powerful framework to eliminate redundancy among asynchronously trained neural networks. 

==> sec/sections/3_method_old.tex <==
\section{Methods}
To reduce the redundancy between models, we first construct joint low rank matrices using weight matrices as blocks, followed with low rank approximation. Specifically, given a set of $M$ neural networks, we first find groups of weight matrices with high similarity. One such group of $N$ weight matrices can be denoted as $\{W_i\in\mathbb{R}^{h\times w}\}_{i=1}^N$. We then construct a joint matrix $J$ by concatenating the weights either column-wise or row-wise. One can also vectorize matrices before concatenation. We then get a parameter-efficient low rank approximation of $J$ with either structured sparse decomposition or singular value decomposition. We now describe details on each step of the process.

\subsection{Joint Matrix Construction}
It is generally hard to find similarity among weight matrices from arbitrary neural networks. Luckily, recent research discovered some useful heuristics in limited settings. Specifically, \textit{linear mode connectivity} (LMC) \citep{frankle2020linear} (might be a derived conclusion) suggests that models fine-tuned from the same pre-trained model have very similar weights. Meanwhile, \textit{permutation symmetries} has also been explored to recover similarity between models with same architecture but trained from different initialization \citep{ainsworth2022git}. 

As a demonstration, we focus on leveraging LMC to compress multiple fine-tunes of a pre-trained model in our study. Specifically, given $N$ models, we group the same layers together. $\{W_i\in\mathbb{R}^{h\times w}\}_{i=1}^N$
Without loss of generality, we use column-wise concatenation without vectorization:
\begin{equation}
    J = [W_1 \quad W_2 \quad \cdots \quad W_N]\in\mathbb{R}^{h\times Nw}
\end{equation}

\subsection{Structured Sparse Decomposition}
Given a set of $N$ weight matrices , model superposition finds a set of $N$ context matrices $\{C_i\in\mathbb{R}^{w\times r}\}_{i=1}^N$ to acquire the superposed weight matrix $W_*$ with $r\in\mathbb{Z}^+$:
\begin{equation} \label{ee1}
W_* = [W_1 \quad W_2 \quad \cdots \quad W_N]
\begin{bmatrix}
C_1 \\
C_2 \\
\vdots \\
C_N
\end{bmatrix} \in \mathbb{R}^{h \times r}
\end{equation}

To retrieve individual weight matrices from $W_*$, model superposition constructs another set of $N$ retrieval matrices $\{R_i\in\mathbb{R}^{r\times w}\}_{i=1}^N$ such that 
$$\forall i\in\{1,\dots,N\},\hat{W}_i=W_*R_i$$

Expanding this for all $i$, we get:
\begin{align} \label{e6}
&\underbrace{[\hat{W}_1 \quad \hat{W}_2 \quad \cdots \quad \hat{W}_N]}_{=\hat{W}\in\mathbb{R}^{h\times Nw}} = W_* [R_1 \quad R_2 \quad \cdots \quad R_N] \nonumber \\
&= \underbrace{[W_1 \quad W_2 \quad \cdots \quad W_N]}_{=W\in\mathbb{R}^{h\times Nw}} 
\underbrace{\begin{bmatrix}
C_1 \\
C_2 \\
\vdots \\
C_N
\end{bmatrix}}_{=C\in\mathbb{R}^{Nw\times r}} \underbrace{[R_1 \quad R_2 \quad \cdots \quad R_N]}_{=R\in\mathbb{R}^{r\times Nw}}\nonumber\\
&= [W_1 \quad W_2 \quad \cdots \quad W_N]
\begin{bmatrix}
C_1R_1 & C_1R_2 & \cdots & C_1R_N \\
C_2R_1 & C_2R_2 & \cdots & C_2R_N \\
\vdots & \vdots & \ddots & \vdots \\
C_NR_1 & C_NR_2 & \cdots & C_NR_N
\end{bmatrix}
\end{align} 
\begin{equation}
    \hat{W} = WCR
\end{equation}
where $WC\in\mathbb{R}^{h\times r}$ and $R\in\mathbb{R}^{r\times Nw}$. Thus, model superposition provides a rank-$r$ approximation of the original matrices $W$. In practice, $r<rank(W)$, and $R$ is a sparse matrix. That makes model superposition a sparse low-rank approximation.

\subsection{Singular Value Decomposition}

One potential downside of SVD is that less significant components might be more important for task accuracy.



% To reduce the redundancy among a set of weight matrices $\{W_i\in \mathbb{R}^{h_i\times w_i}\}_{i=1}^N$, we first partition each matrix into blocks of the same size, and aggregate them into a set of weight blocks $\{B_i\}_{i=1}^M \in \mathbb{R}^{h\times w}$. 


Model merging has drawn significant attention in recent literature due to its unique benefits in combing the capabilities of multiple models into a single set of weights with minimal performance degradation. It is widely assumed that model merging works based on Linear Mode Connectivity (LMC) among the merged checkpoints. This means that linearly interpolating a set of models with LMC will result in the same loss basin (QUESTION: how does LMC explain such endpoint is superior than any other base model?). Although LMC-guided merging methods have increasingly matched the performance of individual fine-tuned models (MAKE THIS PART CLEAR), this assumption has largely restricted the community to focus on merging models with the same architecture or even the same initialization.

To illustrate how MS works, let's (show "retrieval" reformulation and then show it's about interference minimization, LMC is just one special case in this framework, and we can leverage this insight to design a series of techniques to minimize the interference effectively, experiments show the effectiveness of our method, with focus on the claims we make here).



% (MS stands for model superposition).
% bi-MS BMS
% quat-MS QMS

% We are essentially compressing multiple models concurrently with no restriction on model's domain, architecture, and task they are trained for. This has big implication for modular systems like VisProg, ViperGPT, Huggingface and alike. While enjoying the sunshine of LEGOing models in and out to solve combinatorially hard problems with high interpretability, they have notoriously large memory footprint.

% Differentiate between domain and task.

% Lay the foundation for programmatic foundation models' application in robotics where edge device has limited resources while a large amount of primitive neural networks are required for handling diverse real-world situations.

% failure case analysis

% Combination of Vector Symbolic Architectures (VSAs) and model compression might be the way to go.

% Also compressed sensing and quantum physics.


% Two ways 

% Need to prove bounds for ML papers. Method Section Outline: first an empirical problem (e.g., model merging face conflict issue), then explain how you can formulate this into some kind of optimization problem, then solve it, prove some bounds.

% Fields to look into: Discrepancy Minimization, Herding Problem. The Ci will likely be a ring-like structrue at the end. First try to use dummy Ws like Identity matrix and see if I can get such a set of Ci.





\textbf{Interference absorption.} During matrix retrieval, to minimize the interference caused by superposition, we introduce an "absorber" matrix that absorbs most of the interference to enable interference-free collapse for the rest of the matrices. A toy example is as follows: considering four $1\times1$ matrices with the same value $[x]$. We use the following coefficients to put them in superposition: $-2, 1, 1, 1$. Now when retrieving each of them, we receive $0$ interference for the last three matrices, while matrix 1 will get $-\frac{3}{2}[x]$ interference.



Now we show that existing model merging methods can be reformulated into the model store-retrieve framework.


(In previous literature \citet{cheung2019superposition}, the idea is to push weight vectors further apart before superposition to make them cancel each other's out. That's kind of what we did in superposed task arithmetic and it works, but does not work on model soup. We then add the absorber and solved the issue. But the optimal solution seems to doing the exact opposite -- we push all the weight vectors closer and construct carefully the absorber so it absorb most of the interference.) -> 


Algorithm Draft: 

Stage I: Atomic Block Grouping

Need to find atomic blocks that differ by a factor of a scalar. The more similar they are, the more information we can retain with the shared matrix, and the sparser invertible transformation matrices can be.

Option I: Clustering

We first set up the block dimension as hyper-parameters. Then divide up each weight matrix into a set of atomic blocks uniformly. Flatten the blocks into vectors. And use clustering algorithms to get vector clusters.

Option II: Convolution

We first divide up the first weight matrix evenly. For each atomic block, use convolution to find the most similar (factor of a scalar) atomic blocks from the rest of the matrices. Keep doing this until all blocks are assigned.

Stage II: Superposition



Can either subtract common matrix or not. A tradeoff between performance and storage space.


Explore the PEFT perspective -- context as LoRA modules.

Explore superpose PEFT modules (e.g., LoRA).


Strive for simplicity.
